Fully Convolutional Open Set Segmentation

In semantic segmentation knowing about all existing classes is essential to yield effective results with the majority of existing approaches. However, these methods trained in a Closed Set of classes fail when new classes are found in the test phase. It means that they are not suitable for Open Set scenarios, which are very common in real-world computer vision and remote sensing applications. In this paper, we discuss the limitations of Closed Set segmentation and propose two fully convolutional approaches to effectively address Open Set semantic segmentation: OpenFCN and OpenPCS. OpenFCN is based on the well-known OpenMax algorithm, configuring a new application of this approach in segmentation settings. OpenPCS is a fully novel approach based on feature-space from DNN activations that serve as features for computing PCA and multi-variate gaussian likelihood in a lower dimensional space. Experiments were conducted on the well-known Vaihingen and Potsdam segmentation datasets. OpenFCN showed little-to-no improvement when compared to the simpler and much more time efficient SoftMax thresholding, while being between some orders of magnitude slower. OpenPCS achieved promising results in almost all experiments by overcoming both OpenFCN and SoftMax thresholding. OpenPCS is also a reasonable compromise between the runtime performances of the extremely fast SoftMax thresholding and the extremely slow OpenFCN, being close able to run close to real-time. Experiments also indicate that OpenPCS is effective, robust and suitable for Open Set segmentation, being able to improve the recognition of unknown class pixels without reducing the accuracy on the known class pixels.

==> sec_1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

% Remote sensing images and automatic mapping
The development of new technologies for acquisition of aerial images on board satellites or aerial vehicles has made it possible to observe and study various phenomena on the Earth's surface, both on a small and large scale. A highly requested task, in this sense, is automated geographic mapping because it makes easier and faster monitoring cities, regions, countries or entire continents which impacts positively in decision-making.

\begin{figure}[!t]
    \centering
    \includegraphics[clip, trim=0.0cm 1.5cm 0.0cm 0.0cm, width=\textwidth]{figs/Graphical_Abstract_OSR.pdf}
    \caption{Graphical depiction of the problem settings of Closed Set, Anomaly Detection and Open Set Recognition in dense labeling scenarios. The $x$-axis ranges from fully Closed Set (that is, assuming full knowledge of the world) on the left side to Open Set on the rightmost example. In the middle, there is the binary task of Pixel Anomaly Detection, wherein pixels are segmented either into KKCs or UUCs without discerning between distinct KKCs. We also depict the Label Space (Semantic Segmentation map) and a sample of some pixels' representation in a 2D manifold of the Feature Space separated by labels and decision boundaries for each class.}
    \label{fig:problem_setting}
\end{figure}

Automatic mapping from remote sensing images is typically modeled as a supervised classification process, wherein a model is first trained using labeled pixels and then used to classify other pixels in a new region. This process is called semantic segmentation by computer vision community and was severely boosted by a wide number of techniques proposed in the last few years based on convolutional neural networks~\cite{Lateef2019:Neurocomputing}. Indeed, remote sensing applications impose many other challenges that required adaptations or more specific approaches~\cite{Audebert:2016,Kanan2018:IJPRS,Nogueira2019:TGRS,Guiotte2020:GRSL}.

% Classificação e segmentação Open Set
Although semantic segmentation methods have evolved considerably in both Computer Vision and Remote Sensing (RS) applications, some limitations still persist. A case in which the main semantic segmentation methods will fail concerns Open Set scenarios~\cite{Silva:2020}, which deal with the following situation: the model is trained to learn patterns associated with a certain set of classes but in the prediction phase the model is exposed to a set of samples that may be part of unknown classes. In general, a model suitable for Open Set semantic segmentation should be able to indicate in the prediction phase which pixels belong to each class and which ones are not in the set of known classes.

%\todo{Adicionar referências nesse parágrafo...}
It is not strong to say that the world is Open Set when talking about remote sensing applications. We can list a myriad of real situations where Closed Set strategies will fail in semantic segmentation tasks if some class is not clearly indicated in the training and is not present in the predicting phase. For instance, in urban scenes datasets is very common to indicate a fix number of classes and create an extra ``background'' or ``others'' to indicate unknown pixel class or not considered~\cite{maggiori2016high}. Pixels belonging to ``others'' class often lead to bad results and, therefore, it is not uncommon find papers that exclude then from the evaluation metrics computation. Another example is mapping vegetation species such as performed in~\cite{nogueira2017semantic} or ~\cite{nogueira2019spatio}. In~\cite{nogueira2019spatio}, just a very limited number of plant species are indicated in a Savanna Cerrado scene and semantically segment all the scene will certainly lead to a bad result. Because of that, the authors assume a cross-validation protocol that evaluate the proposed method only in a set of know pixel classes. Training semantic segmentation models for remote sensing applications by using Closed Set approaches can also make it difficult to use them in the context of knowledge transfer to different geographical regions. A model for mapping trees by species trained in the Brazilian Amazon, for example, is unlikely to work properly in Peruvian Amazon because of many endemic species. In urban environments, types of buildings present in industrial cities may not exist in a neighboring touristic city.

% Open Set classification in remote sensing
In this paper, we proposed two novel approaches for Open Set semantic segmentation of remote sensing image. We evaluate our methods and compare it with baselines by simulating Open Set situations in well known urban scenes such as Vaihingen and Potsdam datasets.
It is important to mention that the concept of Open Set semantic segmentation is still very little explored in the literature. The first and unique work that introduces this problem is~\cite{Silva:2020}, which proposes a method based on OpenMax~\cite{Bendale:2016} for pixelwise classification, which have many limitations concerning both effectiveness and efficiency.

% Traditional Pattern Recognition tasks assume their knowledge of the world to be complete

%Since the recent advances in the training procedure of Deep Neural Networks (DNNs), feature learning has been the standard practice for state-of-the-art recognition in visual understanding problems. Convolutions were proved to be efficient and allow for high semantic level feature extraction from raw unstructured data in images~\cite{Krizhevsky:2012}. Traditional convolutional architectures are trained in datasets for object classification, as most standard tasks in Computer Visions aim to perform this kind of inference~\cite{Lecun:1998,Krizhevsky:2009,Deng:2009}.

%Traditional Convolutional Neural Networks (CNNs)~\cite{Krizhevsky:2012} were quickly adapted to perform other tasks, including dense labeling, as in object detection~\cite{Girshick:2014,Girshick:2015,Ren:2015}, semantic segmentation~\cite{Long:2015,Ronneberger:2015,Badrinarayanan:2017}, instance segmentation~\cite{He:2017} and video understanding~\cite{Tran:2018}. Other domains also benefited from deep feature learning in images, as biomedical images~\cite{Litjens:2017}, biometrics~\cite{Sundararajan:2018} and remote sensing~\cite{Nogueira:2017}. Semantic Segmentation by DNNs specifically is modeled as a dense classification task~\cite{Long:2015} -- that is, a classification wherein the label of the central pixel from a certain region is used as the classification objective. Fully convolutional training of these networks is shown to improve both accuracy and efficiency of CNNs in dense labeling~\cite{Long:2015}.% and, with time, Encoder-Decoder architectures~\cite{Ronneberger:2015,Badrinarayanan:2017} started being proposed in order to allow for finer details to be modeled in the final prediction map.

%Considering recent advances in satellite data acquisition and cloud computing, access to high-resolution satellite images was facilitated and could be used for solving societal issues~\cite{Gorelick:2017}. The main reason that Remote Sensing (RS) became so important is that this kind of images can provide an overview of vast land areas and can also incorporate additional information from different spectral domains. Thus, a myriad of applications that use CNNs in RS images started to be widely studied, such as natural disaster monitoring~\cite{Nogueira:2018}, urban landuse planning~\cite{Srivastava:2019} and tracking agricultural yields~\cite{Nogueira:2016}.

Within Computer Vision and RS applications, most tasks assume a complete knowledge of the world, hence adopting Closed Set methods for handling their tasks. However, this modelling is highly prone to miss-recognition in real-world data, as many scenarios present classes that are not previously known by the algorithm. These other scenarios can benefit from using Open Set algorithms~\cite{Scheirer:2012}, due to the unforeseeable nature of the images. This holds true for classical visual recognition tasks as object classification/detection~\cite{Bendale:2015,Miller:2018} and action recognition~\cite{Shu:2018} -- and for other applications as well, including RS~\cite{Scherreik:2016,Silva:2020}. Geng \textit{et al.}~\cite{Geng:2020} and Scheirer \textit{et al.}~\cite{Scheirer:2014} describe four sets of classes that the field of Pattern Recognition must consider:
\begin{itemize}
    \item \textbf{Known Known Classes (KKCs)}: positively labeled classes fed in a supervised manner to the model during training. These types of classes are the basis for Closed Set scenarios as % MNIST~\cite{Lecun:1998}, CIFAR~\cite{Krizhevsky:2009} and
    ImageNet~\cite{Deng:2009};
    \item \textbf{Known Unknown Classes (KUCs)}: labeled negative samples, not necessarily clustered into distinct semantics groups. Negatively labeled classes are often not considered in the training procedure due to a lack of interest in their recognition for a specific task, as the case of background classes in segmentation datasets (i.e. Pascal VOC~\cite{Everingham:2015} and COCO~\cite{Lin:2014});
    \item \textbf{Unknown Known Classes (UKCs)}: classes with no available samples during training, but with side information that can be used in training, commonly seen in zero-, one- or few-shot learning~\cite{Palatucci:2009,Zhang:2015,Romera:2015,Vinyals:2016,Snell:2017}; 
    and
    \item \textbf{Unknown Unknown Classes (UUCs)}: classes that completely lack data, labels and additional information about them during training.
\end{itemize}

Based on this taxonomy, traditional Closed Set algorithms for visual understanding are trained to perform inference over KKCs, ignoring KUCs, UKCs and UUCs, which may lead to misrecognition on their deploy. Open Set Recognition (OSR) can be described as the set of algorithms that address the problem of identifying UUCs~\cite{Scheirer:2014} in an unsupervised manner, as there are no data available to do it in supervised or semi-supervised ways. In other words, an Open Set model must be able to identify samples from classes that were not fed to it and possibly not even known during training. Distinctly from Anomaly Detection, where the problem of discriminating between KKCs and UUCs is a simple binary task, OSR aims to degrade the quality of KKC classification as little as possible. Readers should notice that maintaining KKC classification performance and correctly identifying UUCs are often conflicting objectives.

OSR can be achieved via transductive learning~\cite{Li:2005} by trying to infer samples from UUCs using the test data distribution. Another methodology previously proposed for Anomaly Detection that could be used adapted for OSR is the use of auxiliary data to try to learn a generative model via supervision. This is explored in Outlier Exposure (OE)~\cite{Hendrycks:2018}, which yielded competitive results in small classification datasets as MNIST~\cite{Lecun:1998} and CIFAR~\cite{Krizhevsky:2009}. Neither of these approaches is ideal for Open Set semantic segmentation, as transduction requires continuous updates of a model in order to cope with new data, presenting an overhead that might be too expensive in most real-world applications. On the other hand, OE depends on the existence and availability of auxiliary Out-of-Distribution (OOD) data for training, which may not be possible or even useful in semantic segmentation. Therefore, an Open Set semantic segmentation algorithm must rely solely on inductive learning and use only the available training data and KKCs, while also addressing performance concerns, given the higher output dimensions of segmentation.

The main contributions of this work are:
\begin{enumerate}
    \item The first fully convolutional methodology for semantic segmentation in RS imagery or otherwise adapted from OpenMax~\cite{Bendale:2016}, explained in Section~\ref{sec:openfcn};
    \item Proposal of a completely novel fully convolutional methodology for identifying UUCs in dense labeling scenarios using Principal Components from the internal feature space of the DNNs, further described in Section~\ref{sec:openpcs};
    \item Definition of a benchmark evaluation protocol with standard threshold-dependent and threshold-independent metrics for testing OSR Semantic Segmentation tasks;%, as well as presenting guidelines for training such architectures;
    \item Extensive evaluations of architectures and thresholding for the proposed approaches and both Open and Closed Set baselines.
\end{enumerate}.

% The paper also aims to achieve the following objectives: 1) Verify that OpenMax adapts well to a dense labeling task with orders of magnitude fewer classes than a large dataset as ImageNet; % (due to Weibull fitting depending on the output feature vector); 
% 2) Compare the performance of patchwise approaches (i.e. OpenPixel~\cite{Silva:2020}) with fully convolutional training for Open Set Segmentation; 3) Assess the gains of fine-tuning vs. training from scratch, architectural choice and thresholding value among FCN architectures in Open Set Semantic Segmentation of aerial images; 4) Propose a benchmark evaluation protocol for testing Open Set Semantic Segmentation tasks, as well as providing guidelines for training such architectures; 5) Evaluate the scalability of OpenMax in dense labeling.

This paper is organized in sections, as follow: Section \ref{sec:related_work} presents the related work, other papers that try to solve the Open Set semantic segmentation problem; Section \ref{sec:method} describes the proposed methods, explaining in details how it works; 
% Section \ref{sec:evaluation_protocol} explains the proposed evaluation protocol to be used with Open Set semantic segmentation algorithms;
Section \ref{sec:experiments} shows the setup used for this paper, the datasets evaluated and the metrics; Section \ref{sec:results} presents the obtained results from the experimental setup; Finally, section \ref{sec:conclusion} contains the conclusion over the obtained results and the proposed method.
